How To Not Drive: Learning Driving Constraints from Demonstration

We propose a new scheme to learn motion planning constraints from human driving trajectories. Behavioral and motion planning are the key components in an autonomous driving system. The behavioral planning is responsible for high-level decision making required to follow traffic rules and interact with other road participants. The motion planner role is to generate feasible, safe trajectories for a self-driving vehicle to follow. The trajectories are generated through an optimization scheme to optimize a cost function based on metrics related to smoothness, movability, and comfort, and subject to a set of constraints derived from the planned behavior, safety considerations, and feasibility. A common practice is to manually design the cost function and constraints. Recent work has investigated learning the cost function from human driving demonstrations. While effective, the practical application of such approaches is still questionable in autonomous driving. In contrast, this paper focuses on learning driving constraints, which can be used as an add-on module to existing autonomous driving solutions. To learn the constraint, the planning problem is formulated as a constrained Markov Decision Process, whose elements are assumed to be known except the constraints. The constraints are then learned by learning the distribution of expert trajectories and estimating the probability of optimal trajectories belonging to the learned distribution. The proposed scheme is evaluated using NGSIM dataset, yielding less than 1\% collision rate and out of road maneuvers when the learned constraints is used in an optimization-based motion planner.

==> sections/related_work/il.tex <==
\subsection{Imitation Learning}

\subsection{Generative Adversarial Imitation Learning approaches}

In the work of Raunak et al.\cite{bhattacharyya2020modeling} they define the human driving problem as multi-agent, non-linear and stochastic with an unknown cost function. 
They propose 3 modifications to GAIL to solve the formulated driving problem. 
To incorporate multi-agent behavior in learning they propose Parameter-Sharing GAIL by combining GAIL with PS-TRPO which has shared policy parameters. 
With Reward Augmented Imitation Learning they incorporate behavior planning with external penalties whose relative values are defined by the learning task.
They propose Burn-InfoGAIL by excluding the learned embedding layer of InfoGAIL to find the latent variability in the demonstration set. 
They show a comparison with both rule and learning-based methods applied in real driving data.

Junning et al. \cite{huang2019learning} propose a modular framework for adversarial style generative learning with data-driven high-level planning and configurable low-level control. They filter different behaviors into one decision module. The module also supports integration with non-differential
low-level planning or control modules through reparametrized generative adversarial learning.

The method deep mimic [] learns the control policy from simulated characters and their corresponding motion dynamics satisfying certain task boundaries.


==> sections/related_work/il_vs_irl.tex <==
\subsection{IL vs IRL}

IL can be considered as classification which is mimicking the expert's strategy given a set of choices.
It is similar to creating a memory of experts behavior and generalizing it. 
On the other hand, IRL considers expert's policy in MDP and tries retrieve the reward function given some set of expert's demonstration. 
The learned reward best describes the agent's behavior. \cite{7464854_il_irl_link} tries to establish link between IL and IRL finding a common ground in between them.
In their experimental setup, IRL methods do better than IL when a good representation of reward and environment dynamics are 
given. 
In the opposite case, IL does better and generalizes more to unknown situations.
VDB uses an information bottleneck based [] regularizer to minimize the input information by combining GANs with IRL.



==> sections/related_work/irl.tex <==
\subsection{Inverse Reinforcement Learning}

Reinforcement Learning has successfully been used for learning from experiences in the context of sequential decision making games [] , atari games , self-driving cars and many more domains [] . Few of the challenges of RL are the cost of exploration to find the optimal solution and finding am appropriate reward function. Where as Inverse Reinforcement learns the reward function from expert demonstrations. 

One of the applications of IRL is trajectory planning Sacha et al. \cite{rosbach2020planning} use a single reward function for different driving situations. The reward function is computed with path integral MaxEnt-IRL \cite{Aghasadeghi2011MaximumEI} trained from human driving demonstrations in the context of sample-based planning algorithm.
They propose an LSTM based attention deep network that uses a low dimensional context vector of the driving features and actions of sampled-driving policies. They argue the attention vector filters non-human like trajectories.

Another sample-based approach is proposed by \cite{Wu_2020}. 
In this work, a coarse path is created from the samples along the path.
Then smoothed with the kinodynamic of the vehicle.
The planning has two steps with the first step only the path and the second step finding the speed.
The reward is defined as linear-structured with predefined features. The coefficients of the rewards are learned via IRL from the demonstration. 
A similar approach of sampling is also found in \cite{7535466_swerve} for swerving maneuver with static objects on either side of the road. The sampling-based approach is used to find control points for the swerve maneuver and then fit a path that matches the vehicle kinodynamics to the control points.
IRL is used to learn to swerve parameters (control points) from human driving demonstrations.

Use of MaxEnt IRL in modeling behavior of pedestrian and cyclist can be found in \cite{Modeling_pedestrian_cyclist}. 
They combine Maximum Entropy (ME) and Feature Matching(FM) techniques. The MDP is formed with the cyclist as an agent with states composed of distance and speed variables. 
The FM matches the feature count of the expert trajectories. 

RL optimization may be costly, \cite{Accelerated_irl} proposed randomly sample a massive set of policies in advance and the choose one of them as optimal policy. If the sampled policy is not optimal then exploration policy is initiated.

Gabriel et. al \cite{kalweit2020deep} propose a combination IRL and Q-learning. 
They argue that their approaches can learn faster than different variants of MaxEnt IRL and can incorporate additional constraints on agent's behavior even if they might violate in the demonstrations. 
They assume the expert follows a stochastic policy of Boltzmann distribution and predict the "policy that maximizes the entropy over actions locally at each step as an approximation" which they refer as Inverse action-value Iteration (IAVI). 
They solve the reward function from the system of linear equations formed by the observed transitions. 
They extend this formulation with count-based policy approximation to update tabular Q values. 
For the continuous state space, the reward function is estimated with a neural network. 
In their Deep Constrained IRL, they put a threshold-based constraint on the action space of the demonstrations and learn the new policy. 
The experiments/comparisons are done in Objectworld Benchmark and SUMO simulator with the task of the lane change.


In the work of Maximilian et al. \cite{9196795}, they find suitable cost functions that correspond to human driving behavior. 
They propose different scenarios based on a cost function that is dependant on different driving tasks, time, and driving performance. 
They learn from demonstration with IRL using a particular cost function. 
They propose trajectory selection with the cost functions instead of using the whole set. 
The selection criteria are based on selecting the segments of the data that end in the optimal time stamp. 
Their experiments include in-lane, right turning, and stopping scenarios.

 In \cite{ld_style}, they address the problem of learning a small segment of human driving style on the highway. They extract scalar features similar to cost function from the expert trajectories. 
 Properties such as distance between the vehicles, proper acceleration, jerk are used to define the features. Learning is done in this feature space using MaxEnt IRL.
 The cost function is defined as a linear sum of these features with corresponding coefficients.
 For a given set of demonstrations, the distance between the resulting trajectory and demonstrated trajectory is minimized.
 
 Chou et al. \cite{Chou_2020} propose a search-based approach to find lower cost trajectories that do not violate the known constraints. 
 It is an alternate/"complementary"  solution to recover the latent constraints found within expert demonstration which are shared across multiple tasks.
 The demonstration set needs to have a boundedly-suboptimal cost that satisfies all the constraints. 
 It can learn also learn from the sub-optimal demonstration.
 Although they show collision avoidance in 2D space but their method is unable to work for complex constraint representation.
 
 In the work of \cite{huang2018learning}, they formulate the expert learning as maxmin problem in the RL setup with MDP. 
 The agent chooses a policy and an adversary chooses a reward function that is consistent with the agent’s current knowledge and minimizes the agent’s reward. 
 The goal of the agent is to learn a policy that maximizes the worst possible reward using ellipsoid method and another solution using follow the perturbed-leader method \cite{KALAI2005291}.
 
Driving can be uncertain due to the presence of sensor noise, occlusion, and unknown intention of dynamic objects in the environment.
\cite{8814223_mpc_irl} consider human driver/pedestrian as distributed sensors and observe their behavior and infer the state of the environment
from it. The predicted beliefs are modeled as probabilistic planning with MPC whose cost function is parameterized as a linear combination of features and learned via IRL from demonstrations. 
In this work\cite{YOU20191}, they model driving with MDP which is consistent with any number of lanes and road curvature. 
They use both RL and IRL to show multiple driving behaviors.
At first, an expert agent is trained using RL against a known reward function. 
The trained expert agent is later used to generate demonstrations and the DNN based reward is extracted from demonstrations using IRL approach
by maximizing the entropy of the joint distribution over a short data segment.


\cite{sierragonzalez:hal-01396047} use offline demonstration under MaxEnt IRL for predicting the actions of each of the participating vehicles on the highway. The proposed driver model is formed as linear feature-based
cost function which is used to predict the future dynamics in the future timestamp.


\subsection{IRL for constraints}
An expert agent's behavior is often guided by some constraints.
\cite{scobee2020maximum} try to estimate the underlying constraints using MaxEnt IRL framework's probability distribution over trajectories to retrieve the constraints. 
They find the frequency of occurring a trajectory in the observed set and then iteratively select the individual minimal constraint sets with a proper stopping function. 
Another approach is to use greedy heuristic search where an estimated constraint set is formed
with augmenting it to the final set which covers "the most of the uncovered probability mass". They showed this for deterministic
MDP in 2D collision avoidance problem.


Usman et al. \cite{anwar2020inverse} extend the above work for continuous setting without the consideration of the environment dynamics. They eliminate the state-action space by replacing it with Neural approximating function. The policy is a unconstrained min-max problem in form of the Lagrangian object function. They also add importance sampling on the samples drawn from the policy. They run experiment on environment like reaching a goal in 2D and OpenAI gym 3D motion of Half-Cheetah and Walker.

The method T-REX can learn the desired tasks even with sub optimal demonstrations. They have showed that combining with DRL learns meaningful reward function and has capabilities to outperform the initial trajectory distribution.


==> sections/related_work/others.tex <==
\subsection{Others}
\subsection{Self Play}
Learning from failures can be challenging.
In \cite{sinha2020formulazero}, the authors propose a self-play method that uses distributionally robust bandit optimization for online opponent-modeling with uncertainty in beliefs. 
The approach does not require any demonstration.
They iteratively parameterize other competing agents with population-based synthesis using replica-exchange 
Markov chain Monte Carlo. 
The learned policy applied to both simulation and real robot cars can show Formula One-style racing capability.
MetaMimic uses memory based approach to learn large network and introduces the idea of one-shot high fidelity imitation in the context of RL and IL.


